The Circular Polarization of Sagittarius A* at Submillimeter Wavelengths

We report the first detections of circularly polarized emission at submillimeter wavelengths from the compact radio source and supermassive black hole candidate Sgr A* at a level of 1.2\pm0.3% at 1.3 mm wavelength (230 GHz) and 1.6\pm0.3% at 860 microns (345 GHz) with the same handedness as observed at lower frequencies (1.4-15 GHz). The observations, taken with the Submillimeter Array in multiple epochs, also show simultaneous linear polarization (LP) at both wavelengths of about 6%. These properties differ sharply from those at wavelengths longer than 1 cm (frequencies below 30 GHz), where weak circular polarization (CP) (~ 0.5%) dominates over LP, which is not detected at similar fractional limits. We describe an extensive set of tests to ensure the accuracy of our measurements. We find no CP in any other source, including the bright quasar 1924-292, which traces the same path on the sky as Sgr A* and therefore should be subject to identical systematic errors originating in the instrument frame. Since a relativistic synchrotron plasma is expected to produce little CP, the observed CP is probably generated close to the event horizon by the Faraday conversion process. We use a simple model to show that the phase shift associated with Faraday conversion can be nearly independent of frequency, a sufficient condition to make the handedness of CP independent of frequency. Because the size of the tau=1-surface changes by more than an order of magnitude between 1.4 and 345 GHz, the magnetic field must be coherent over such scales to consistently produce left CP.

==> tab_tracks.tex <==
\renewcommand{\thefootnote}{\alph{footnote}}
\begin{table}[hb] 
%\tabletypesize{\scriptsize}
\caption{Observation Epochs} 
\centering
\begin{tabular}{l r r c r} 
\tableline\tableline
Date  & Main    & Freq.\tablenotemark{a}  & SMA     &$\tau_\mathrm{225\,GHz}$  \\
& Target    &[GHz]  & Config.\tablenotemark{b}      & \\
\tableline 
2005 June 6&Sgr~A*&343.0&CN&0.055 \\
2006 July 17&Sgr~A*&226.9&VEX&0.05-0.08 \\
2007 March 31&Sgr~A*&226.9&CN& 0.055 \\
2008 May 30&1924-292&226.9&CN&0.08 \\
\tableline
\footnotetext[1]{Frequency of the local oscillator. Upper and lower sidebands are centered 5 GHz above and below this frequency, respectively.}
\footnotetext[2]{Array configurations include ``Compact North" (CN) and ``Very Extended" (VEX).}
\end{tabular} 
\label{tab:tracks}
\end{table} 
\renewcommand{\thefootnote}{\arabic{footnote}}


